Privacy-preserving Multi-biometric Indexing based on Frequent Binary Patterns

The development of large-scale identification systems that ensure the privacy protection of enrolled subjects represents a major challenge. Biometric deployments that provide interoperability and usability by including efficient multi-biometric solutions are a recent requirement. In the context of privacy protection, several template protection schemes have been proposed in the past. However, these schemes seem inadequate for indexing (workload reduction) in biometric identification systems. More specifically, they have been used in identification systems that perform exhaustive searches, leading to a degradation of computational efficiency. To overcome these limitations, we propose an efficient privacy-preserving multi-biometric identification system that retrieves protected deep cancelable templates and is agnostic with respect to biometric characteristics and biometric template protection schemes. To this end, a multi-biometric binning scheme is designed to exploit the low intra-class variation properties contained in the frequent binary patterns extracted from different types of biometric characteristics. Experimental results reported on publicly available databases using state-of-the-art Deep Neural Network (DNN)-based embedding extractors show that the protected multi-biometric identification system can reduce the computational workload to approximately 57\% (indexing up to three types of biometric characteristics) and 53% (indexing up to two types of biometric characteristics), while simultaneously improving the biometric performance of the baseline biometric system at the high-security thresholds. The source code of the proposed multi-biometric indexing approach together with the composed multi-biometric dataset, will be made available to the research community once the article is accepted.

==> tables/closed_set_most_ranked_codes.tex <==
\begin{adjustbox}{max width=\linewidth}
    \begin{threeparttable}
    \begin{tabular}{ccccccccccc}
    \toprule
        \textbf{Combination}& \textbf{Approach} & \textbf{k} & \textbf{\#Comb} & \textbf{\#Comp} & \textbf{Std\_comp} & \textbf{W$_u$(\%)} & \textbf{W$_l$(\%)} & \textbf{\#Visited-patterns} &\textbf{Std\_bins\_v}& \textbf{H-R} \\ \cmidrule{1-11}
         \multirow{6}{*}{Face-Fingerprint}&\multirow{24}{*}{Baseline}&3&8&468.57 & 264.51 &72.73&46.48&2.96 & 2.03&100.00\\
                                          &                         &4&16&394.93 & 260.38& 65.01&39.18&5.53 & 4.12 &100.00  \\
                                          &                         &5&32&355.85 & 257.08 &60.80 & 35.30 &10.15 & 8.15 & 99.99  \\
                                          &                         &6&64& 340.12 & 260.56 & 59.59 &  33.74 &19.65 & 16.55 &  99.47  \\
                                          &                         &7&128&332.79 & 254.12 &58.23 & 33.01 & 38.80 & 33.27 & 89.56\\
                                          &                         &8&256& 231.27 & 130.26 &  35.87 &  22.94 & 54.35 & 35.08& 54.95\\ \cmidrule{3-11}

        \multirow{6}{*}{Iris-Fingerprint}&                          &3& 8& 443.98 & 260.32 &69.87 & 44.05 & 2.85 & 1.99 & 100.00   \\
                                          &                         &4&16 & 364.01 & 253.13 & 61.22 &  36.11 &5.15 &3.99 & 100.00 \\
                                          &                         &5&32& 330.72 & 251.67 & 57.78 & 32.81 & 9.49 & 7.92 & 100.00     \\
                                          &                         &6&64& 307.02 & 247.93 & 55.05 & 30.46 & 17.73 & 15.54 & 99.72   \\
                                          &                         &7&128& 307.88 & 250.00 & 55.35 & 30.54 & 35.55 & 32.35 & 91.57 \\
                                          &                         &8&256& 216.20 & 133.31 & 34.67 & 21.45 & 50.76 & 35.53 &  59.49   \\ \cmidrule{3-11}



     \multirow{6}{*}{Face-Iris}&                                    &3&8&  512.58 & 276.62 & 78.29 &  50.85 &  3.46 & 2.19 & 100.00    \\
                                          &                         &4&16 & 454.31  & 277.26 & 72.58 &  45.07 & 6.70 & 4.44 & 100.00 \\
                                          &                         &5&32& 433.38 & 283.41& 71.11 &  42.99 &  13.03 & 9.15 &  99.24  \\
                                          &                         &6&64& 422.60 & 285.52 & 70.25 & 41.92 &  25.450 & 18.33 & 99.97   \\
                                          &                         &7&128& 410.60 & 265.99 & 67.12 & 40.73 &  49.55 & 35.18 & 86.05  \\
                                          &                         &8&256& 261.73 & 115.78 & 37.45 &  25.96 & 64.17  & 31.81 & 43.23     \\ \cmidrule{3-11}

                                          
     \multirow{6}{*}{Face-Fingerprint-Iris}&                        &3&8& 474.58 & 267.71 & 73.64 &  47.08 &  3.13 & 2.09 & 100.00   \\
                                          &                         &4&16 &  403.53 & 267.89 &66.61 & 40.03 & 5.86 & 4.26 & 100.00  \\
                                          &                         &5&32& 368.78 & 265.02 & 62.88 &36.59 & 10.75 & 8.38 &  99.08   \\
                                          &                         &6&64& 365.12 & 267.47 & 62.76 &36.22 &  21.11 & 16.78 & 99.96  \\
                                          &                         &7&128& 351.96 & 251.22 & 59.84 &34.92 & 40.97 & 32.94 & 83.39    \\
                                          &                         &8&256& 166.22 & 74.26 & 23.86 & 16.49 &  39.68 & 19.39 & 34.42    \\ \cmidrule{1-11}


   \multirow{6}{*}{Face-Fingerprint}&\multirow{24}{*}{BioHashing}   &3&8& 493.10 & 260.53 & 74.77 &48.92 & 2.90 & 1.96 & 100.00   \\
                                          &                         &4&16& 383.74 & 258.33 & 63.70  & 38.07 & 5.36 & 3.95 & 100.00 \\
                                          &                         &5&32& 331.37 & 246.72 & 57.35 & 32.87 &  9.46 & 7.53 & 100.00\\
                                          &                         &6&64&  312.80 & 247.64 &  55.60 & 31.03 & 17.31 & 14.80 & 99.72  \\
                                          &                         &7&128& 313.66 & 256.36 & 56.55 & 31.12 & 33.38 & 31.21 &  91.70\\
                                          &                         &8&256&  237.60 & 152.52 & 38.70 & 23.57 &  48.98 & 36.01 &  61.50   \\ \cmidrule{3-11}



        \multirow{6}{*}{Iris-Fingerprint}&                          &3& 8& 476.88 & 255.72 & 72.68 & 47.31 & 2.76 & 1.91 & 100.00   \\
                                          &                         &4&16 & 363.95 & 255.67 & 61.47 & 36.11 &  5.02 & 3.88 & 100.00 \\
                                          &                         &5 & 32 & 311.60 & 243.14 & 55.03 & 30.91 & 8.78 & 7.36 & 100.00    \\
                                          &                         &6&64& 287.23 & 236.06 & 51.91 & 28.50 & 15.73  & 13.98 &  99.73      \\
                                          &                         &7&128& 286.75 & 249.71 & 53.22 & 28.45 & 30.06 & 29.86 & 93.65  \\
                                          &                         &8&256& 226.82 & 155.96 & 37.97 & 22.50 & 46.20 & 36.43 & 64.62  \\ \cmidrule{3-11}


     \multirow{6}{*}{Face-Iris}&                                    &3&8& 531.98 & 281.86 &  80.74 & 52.78 &3.64 & 2.28 & 100.00      \\
                                          &                         &4&16 & 478.46 & 280.50 & 75.29 & 47.47 &  7.18 & 4.52 & 100.00 \\
                                          &                         &5&32& 449.19 & 283.99 & 72.74 &  44.56 & 13.76 & 9.11 & 100.00 \\
                                          &                         &6&64& 437.91 & 285.88 & 71.80 & 43.44 & 26.83 & 18.38 & 99.28      \\
                                          &                         &7&128& 424.86 & 267.69 & 68.71 &  42.15 & 51.78 & 35.17 & 86.32 \\
                                          &                         &8&256& 267.15 & 115.05 & 37.92 & 26.50 & 65.82 & 31.76 &  42.74    \\ \cmidrule{3-11}



                                          
     \multirow{6}{*}{Face-Fingerprint-Iris}&                        &3&8&499.24 & 268.09 & 76.12 &49.53 & 3.16 & 2.10 & 100.00 \\
                                          &                         &4&16 & 408.68 & 268.47 & 67.18 & 40.54 &5.84 & 4.18 & 100.00 \\
                                          &                         &5&32& 367.51 & 259.97 &62.25 & 36.46 & 10.67 & 8.02 & 100.00  \\
                                          &                         &6&64& 349.82 & 262.88 &60.78 & 34.70 & 19.80 & 15.99 & 99.43  \\
                                          &                         &7&128& 337.37 & 256.65 &  58.93 &33.47 & 38.00 & 32.00 & 86.71  \\
                                          &                         &8&256&  179.98 & 82.90 & 26.08 & 17.85 & 39.28 & 20.33 & 37.37     \\ \cmidrule{1-11}     


                                          
   \multirow{6}{*}{Face-Fingerprint}&\multirow{24}{*}{IoM-GRP}      &3&8& 499.07 & 260.94 & 75.40 & 49.51 &  2.80 & 1.94 & 100.00       \\
                                          &                         &4&16& 439.98 &  260.40 & 69.48 &43.65 &4.75 & 3.81 & 100.00  \\
                                          &                         &5&32& 389.56 & 254.10 &  63.85 & 38.65 &8.43 & 7.27& 100.00 \\
                                          &                         &6&64& 354.93 & 247.04 & 59.72 & 35.21 &15.64 & 13.98 & 100.00      \\
                                          &                         &7&128& 331.16 & 241.98 & 56.86 &32.85 & 30.14 & 27.23 & 99.41   \\
                                          &                         &8&256& 303.24 & 239.92 & 53.88& 30.08 & 56.64 & 54.00 & 99.98    \\ \cmidrule{3-11}




        \multirow{6}{*}{Iris-Fingerprint}&                          &3& 8& 476.04 & 255.34 & 72.56 & 47.23 &2.58 & 1.87 & 100.00     \\
                                          &                         &4&16 & 406.76 & 253.44 & 65.50 & 40.35 & 4.44 & 3.72 & 100.00  \\
                                          &                         &5 & 32 & 355.77 & 241.73 &59.28 & 35.29 &  7.63 & 6.90 & 100.00   \\
                                          &                         &6&64& 318.98 & 238.15 & 55.27 & 31.64 & 14.05 & 13.35 & 100.00      \\
                                          &                         &7&128& 294.95 & 235.50 & 52.62 & 29.26 & 26.80 & 26.42 & 100.00   \\
                                          &                         &8&256& 275.50 & 233.84 & 50.53 &  27.33 & 51.51 & 52.19 &99.64  \\ \cmidrule{3-11}




     \multirow{6}{*}{Face-Iris}&                                    &3&8&  515.87 & 278.99 &  78.86 &  51.18 & 3.48 & 2.22 & 100.00     \\
                                          &                         &4&16 & 454.99 & 281.78 & 73.09 &  45.14 &  6.68 & 4.60 & 100.00\\
                                          &                         &5&32& 439.28 & 283.04 & 71.66 & 43.58 &13.25 & 9.19 & 100.00  \\
                                          &                         &6&64& 423.42 & 282.27 & 70.01 & 42.01 & 26.06 & 18.13 & 100.00   \\
                                          &                         &7&128& 422.17 & 284.60 & 70.12 & 41.88 & 51.90 & 36.58 & 100.00  \\
                                          &                         &8&256& 430.86 & 287.75 & 71.29 & 42.74 & 105.33 & 73.94 & 99.10    \\ \cmidrule{3-11}





                                          
     \multirow{6}{*}{Face-Fingerprint-Iris}&                        &3&8& 498.55 & 266.69 & 75.92 & 49.46 & 3.12 & 2.16 &100.00 \\
                                          &                         &4&16 &  433.85 & 262.62 & 69.09 & 43.04 & 5.31 & 4.14 & 100.00  \\
                                          &                         &5&32& 387.48 & 263.67 & 64.60 & 38.44 & 9.59 & 8.08 & 100.00    \\
                                          &                         &6&64&361.49 & 260.48 &  61.70 & 35.86 & 18.39 & 15.76 & 100.00 \\
                                          &                         &7&128& 344.41 & 255.47 & 59.51 & 34.17 & 35.31 & 30.50 & 99.98  \\
                                          &                         &8&256&337.05 & 258.33 & 59.07 & 33.44 & 69.59 & 61.75 &99.98 \\   

    \bottomrule
	\end{tabular}
		\begin{tablenotes}
  \item $k$: Length of the frequent binary pattern, \#Comb: Number of possible combinations to be generated given a $k$, \#Comp: Average number of comparisons, Std\_comp: Standard deviation across the number of comparisons carried out per subject, W$_l$: Lower bound of the computational workload reduction estimated on the average number of comparisons computed per subject, W$_u$: Upper bound of the computational workload reduction, \#Visited-patterns: Average number of binary patterns visited from the probe, Std\_bins\_v: Standard deviation across the bins visited per subject, H-R: Hit-Rate.
  \end{tablenotes}
	\end{threeparttable}
	\end{adjustbox}


==> tables/description_cancelable_btp.tex <==
\begin{adjustbox}{max width=\textwidth}
			  \begin{threeparttable}

	 \begin{tabular}{c c c c c c  } \toprule
		 \textbf{BTP scheme} & \textbf{Input} & \textbf{Length\_i} &  \textbf{Output} & \textbf{Length\_o} &\textbf{\shortstack{Binarisation \\ required}} \\ \midrule

        BioHashing~\cite{Jin-BioHashing-2004}&float&512&binary&512&\xmark\\

        IoM-GRP~\cite{Jin-index-of-hashing-2017}&float&512&integer&2,048&\cmark\\


   	\bottomrule
	\end{tabular}
		\begin{tablenotes}
  \item Length\_i: length of the embedding to be protected, corresponding to the Input. Length\_o: length of the output representations prior to the process of frequent binary pattern extraction.
  \end{tablenotes}
	\end{threeparttable}
	\end{adjustbox}

==> tables/statistics_feature-level_open_set.tex <==


\begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{cccccc}
    \toprule
        Biometric-characteristic & Approach & Combination & P-R & EER & FPIR \\ \cmidrule{1-6}

        face & baseline & FA-FP & 0 & 16.0 & 31.0 \\ \hline
        face & baseline & FA-IR & 0 & 22.0 & 41.0 \\ \hline
        face & baseline & FP-FA & 0 & 17.0 & 32.0 \\ \hline
        face & baseline & IR-FA & 0 & 22.0 & 40.0 \\ \hline
        face & baseline & FA-FP-IR & 0 & 17.0 & 31.0 \\ \hline
        face & baseline & FA-IR-FP & 0 & 17.0 & 34.0 \\ \hline
        face & baseline & FP-FA-IR & 0 & 17.0 & 33.0 \\ \hline
        face & baseline & FP-IR-FA & 0 & 17.0 & 32.0 \\ \hline
        face & baseline & IR-FA-FP & 0 & 18.0 & 34.0 \\ \hline
        face & baseline & IR-FP-FA & 0 & 17.0 & 32.0 \\ \hline
        face & biohashing & FA-FP & 0 & 15.0 & 30.0 \\ \hline
        face & biohashing & FA-IR & 0 & 16.0 & 31.0 \\ \hline
        face & biohashing & FP-FA & 0 & 15.0 & 30.0 \\ \hline
        face & biohashing & IR-FA & 0 & 17.0 & 31.0 \\ \hline
        face & biohashing & FA-FP-IR & 0 & 17.0 & 36.0 \\ \hline
        face & biohashing & FA-IR-FP & 0 & 16.0 & 30.0 \\ \hline
        face & biohashing & FP-FA-IR & 0 & 16.0 & 31.0 \\ \hline
        face & biohashing & FP-IR-FA & 0 & 15.0 & 32.0 \\ \hline
        face & biohashing & IR-FA-FP & 0 & 16.0 & 28.99 \\ \hline
        face & biohashing & IR-FP-FA & 0 & 16.0 & 31.0 \\ \hline
        face & grp & FA-FP & 0 & 15.0 & 28.00 \\ \hline
        face & grp & FA-IR & 0 & 17.0 & 33.0 \\ \hline
        face & grp & FP-FA & 0 & 15.0 & 27.0 \\ \hline
        face & grp & IR-FA & 0 & 17.0 & 31.0 \\ \hline
        face & grp & FA-FP-IR & 0 & 16.0 & 28.00 \\ \hline
        face & grp & FA-IR-FP & 0 & 16.0 & 27.0 \\ \hline
        face & grp & FP-FA-IR & 0 & 16.0 & 30.0 \\ \hline
        face & grp & FP-IR-FA & 0 & 15.0 & 28.00 \\ \hline
        face & grp & IR-FA-FP & 0 & 15.0 & 28.00 \\ \hline
        face & grp & IR-FP-FA & 0 & 16.0 & 30.0 \\ \hline
        fingerprint & baseline & FA-FP & 0 & 18.0 & 28.99 \\ \hline
        fingerprint & baseline & FP-FA & 0 & 20.0 & 34.0 \\ \hline
        fingerprint & baseline & FP-IR & 0 & 17.0 & 28.00 \\ \hline
        fingerprint & baseline & IR-FP & 0 & 18.0 & 30.0 \\ \hline
        fingerprint & baseline & FA-FP-IR & 0 & 19.0 & 33.0 \\ \hline
        fingerprint & baseline & FA-IR-FP & 0 & 19.0 & 28.99 \\ \hline
        fingerprint & baseline & FP-FA-IR & 0 & 18.0 & 28.99 \\ \hline
        fingerprint & baseline & FP-IR-FA & 0 & 19.0 & 30.0 \\ \hline
        fingerprint & baseline & IR-FA-FP & 0 & 19.0 & 34.0 \\ \hline
        fingerprint & baseline & IR-FP-FA & 0 & 19.0 & 31.0 \\ \hline
        fingerprint & biohashing & FA-FP & 0 & 16.0 & 43.0 \\ \hline
        fingerprint & biohashing & FP-FA & 0 & 17.0 & 38.0 \\ \hline
        fingerprint & biohashing & FP-IR & 0 & 18.0 & 46.0 \\ \hline
        fingerprint & biohashing & IR-FP & 0 & 18.0 & 40.0 \\ \hline
        fingerprint & biohashing & FA-FP-IR & 0 & 19.0 & 42.0 \\ \hline
        fingerprint & biohashing & FA-IR-FP & 0 & 19.0 & 39.0 \\ \hline
        fingerprint & biohashing & FP-FA-IR & 0 & 18.0 & 47.0 \\ \hline
        fingerprint & biohashing & FP-IR-FA & 0 & 19.0 & 40.0 \\ \hline
        fingerprint & biohashing & IR-FA-FP & 0 & 18.0 & 39.0 \\ \hline
        fingerprint & biohashing & IR-FP-FA & 0 & 19.0 & 42.0 \\ \hline
        fingerprint & grp & FA-FP & 0 & 16.0 & 27.0 \\ \hline
        fingerprint & grp & FP-FA & 0 & 17.0 & 27.0 \\ \hline
        fingerprint & grp & FP-IR & 0 & 15.0 & 26.0 \\ \hline
        fingerprint & grp & IR-FP & 0 & 16.0 & 25.0 \\ \hline
        fingerprint & grp & FA-FP-IR & 0 & 18.0 & 34.0 \\ \hline
        fingerprint & grp & FA-IR-FP & 0 & 17.0 & 28.99 \\ \hline
        fingerprint & grp & FP-FA-IR & 0 & 17.0 & 26.0 \\ \hline
        fingerprint & grp & FP-IR-FA & 0 & 17.0 & 28.00 \\ \hline
        fingerprint & grp & IR-FA-FP & 0 & 17.0 & 27.0 \\ \hline
        fingerprint & grp & IR-FP-FA & 0 & 18.0 & 28.00 \\ \hline
        iris & baseline & FA-IR & 0 & 27.0 & 59.0 \\ \hline
        iris & baseline & IR-FA & 0 & 27.0 & 56.99 \\ \hline
        iris & baseline & FP-IR & 0 & 20.0 & 47.0 \\ \hline
        iris & baseline & IR-FP & 0 & 20.0 & 47.0 \\ \hline
        iris & baseline & FA-FP-IR & 0 & 17.0 & 31.0 \\ \hline
        iris & baseline & FA-IR-FP & 0 & 17.0 & 34.0 \\ \hline
        iris & baseline & FP-FA-IR & 0 & 17.0 & 33.0 \\ \hline
        iris & baseline & FP-IR-FA & 0 & 17.0 & 32.0 \\ \hline
        iris & baseline & IR-FA-FP & 0 & 18.0 & 34.0 \\ \hline
        iris & baseline & IR-FP-FA & 0 & 17.0 & 32.0 \\ \hline
        iris & biohashing & FA-IR & 0 & 30.0 & 61.0 \\ \hline
        iris & biohashing & IR-FA & 0 & 30.0 & 62.0 \\ \hline
        iris & biohashing & FP-IR & 0 & 20.0 & 50.0 \\ \hline
        iris & biohashing & IR-FP & 0 & 20.0 & 48.0 \\ \hline
        iris & biohashing & FA-FP-IR & 0 & 17.0 & 36.0 \\ \hline
        iris & biohashing & FA-IR-FP & 0 & 16.0 & 30.0 \\ \hline
        iris & biohashing & FP-FA-IR & 0 & 16.0 & 31.0 \\ \hline
        iris & biohashing & FP-IR-FA & 0 & 15.0 & 32.0 \\ \hline
        iris & biohashing & IR-FA-FP & 0 & 16.0 & 28.99 \\ \hline
        iris & biohashing & IR-FP-FA & 0 & 16.0 & 31.0 \\ \hline
        iris & grp & FA-IR & 0 & 22.0 & 48.0 \\ \hline
        iris & grp & IR-FA & 0 & 32.0 & 68.0 \\ \hline
        iris & grp & FP-IR & 0 & 18.0 & 48.0 \\ \hline
        iris & grp & IR-FP & 0 & 19.0 & 48.0 \\ \hline
        iris & grp & FA-FP-IR & 0 & 16.0 & 28.00 \\ \hline
        iris & grp & FA-IR-FP & 0 & 16.0 & 27.0 \\ \hline
        iris & grp & FP-FA-IR & 0 & 16.0 & 30.0 \\ \hline
        iris & grp & FP-IR-FA & 0 & 15.0 & 28.00 \\ \hline
        iris & grp & IR-FA-FP & 0 & 15.0 & 28.00\\ \hline
        iris & grp & IR-FP-FA & 0 & 16.0 & 30.0 \\ 


      \bottomrule
     \end{tabular}
     \end{adjustbox}

==> tables/statistics_representation-level_open_set.tex <==

\begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{cccccc}
    \toprule
        \textbf{Biometric-characteristic} &\textbf{Approach} &\textbf{Combination} & \textbf{P-R(in\%)}& \textbf{EER(in\%)} & \textbf{FPIR0.1(in\%)}\\ \cmidrule{1-6}
        face & baseline & FA-FP & 0 & 19.0 & 36.0 \\ 
        face & baseline & FA-IR & 0 & 19.0 & 35.0 \\ 
        face & baseline & FP-FA & 0 & 14.00 & 30.0 \\ 
        face & baseline & IR-FA & 0 & 18.0 & 34.0 \\ 
        face & baseline & FA-FP-IR & 0 & 19.0 & 38.0 \\ 
        face & baseline & FA-IR-FP & 0 & 21.0 & 38.0 \\ 
        face & baseline & FP-FA-IR & 0 & 20.0 & 38.0 \\ 
        face & baseline & FP-IR-FA & 0 & 21.0 & 39.0 \\ 
        face & baseline & IR-FA-FP & 0 & 20.0 & 37.0 \\ 
        face & baseline & IR-FP-FA & 0 & 20.0 & 36.0 \\ 
        face & biohashing & FA-FP & 0 & 19.0 & 38.0 \\ 
        face & biohashing & FA-IR & 0 & 16.0 & 30.0 \\ 
        face & biohashing & FP-FA & 0 & 18.0 & 33.0 \\ 
        face & biohashing & IR-FA & 0 & 16.0 & 31.0 \\ 
        face & biohashing & FA-FP-IR & 0 & 17.0 & 34.0 \\ 
        face & biohashing & FA-IR-FP & 0 & 17.0 & 34.0 \\ 
        face & biohashing & FP-FA-IR & 0 & 19.0 & 35.0 \\ 
        face & biohashing & FP-IR-FA & 0 & 17.0 & 32.0 \\ 
        face & biohashing & IR-FA-FP & 0 & 18.0 & 35.0 \\ 
        face & biohashing & IR-FP-FA & 0 & 17.0 & 33.0 \\ 
        face & grp & FA-FP & 0 & 19.0 & 34.0 \\ 
        face & grp & FA-IR & 0 & 13.0 & 25.0 \\ 
        face & grp & FP-FA & 0 & 15.0 & 30.0 \\ 
        face & grp & IR-FA & 0 & 14.00 & 27.0 \\ 
        face & grp & FA-FP-IR & 0 & 13.0 & 26.0 \\ 
        face & grp & FA-IR-FP & 0 & 15.0 & 28.00\\ 
        face & grp & FP-FA-IR & 0 & 16.0 & 28.99 \\ 
        face & grp & FP-IR-FA & 0 & 15.0 & 27.0 \\ 
        face & grp & IR-FA-FP & 0 & 16.0 & 28.00 \\ 
        face & grp & IR-FP-FA & 0 & 13.0 & 26.0 \\ 
        fingerprint & baseline & FA-FP & 0 & 19.0 & 31.0 \\ 
        fingerprint & baseline & FP-FA & 0 & 18.0 & 31.0 \\ 
        fingerprint & baseline & FP-IR & 0 & 20.0 & 35.0 \\ 
        fingerprint & baseline & IR-FP & 0 & 21.0 & 37.0 \\ 
        fingerprint & baseline & FA-FP-IR & 0 & 20.0 & 37.0 \\ 
        fingerprint & baseline & FA-IR-FP & 0 & 22.0 & 36.0 \\ 
        fingerprint & baseline & FP-FA-IR & 0 & 20.0 & 36.0 \\ 
        fingerprint & baseline & FP-IR-FA & 0 & 23.0 & 36.0 \\ 
        fingerprint & baseline & IR-FA-FP & 0 & 20.0 & 33.0 \\ 
        fingerprint & baseline & IR-FP-FA & 0 & 21.0 & 37.0 \\ 
        fingerprint & biohashing & FA-FP & 0 & 21.0 & 50.0 \\ 
        fingerprint & biohashing & FP-FA & 0 & 18.0 & 38.0 \\ 
        fingerprint & biohashing & FP-IR & 0 & 19.0 & 42.0 \\ 
        fingerprint & biohashing & IR-FP & 0 & 18.0 & 41.0 \\ 
        fingerprint & biohashing & FA-FP-IR & 0 & 18.0 & 48.0 \\ 
        fingerprint & biohashing & FA-IR-FP & 0 & 21.0 & 38.0 \\ 
        fingerprint & biohashing & FP-FA-IR & 0 & 18.0 & 41.0 \\ 
        fingerprint & biohashing & FP-IR-FA & 0 & 17.0 & 36.0 \\ 
        fingerprint & biohashing & IR-FA-FP & 0 & 18.0 & 35.0 \\ 
        fingerprint & biohashing & IR-FP-FA & 0 & 19.0 & 39.0 \\ 
        fingerprint & grp & FA-FP & 0 & 15.0 & 28.00 \\ 
        fingerprint & grp & FP-FA & 0 & 19.0 & 28.99 \\ 
        fingerprint & grp & FP-IR & 0 & 16.0 & 26.0 \\ 
        fingerprint & grp & IR-FP & 0 & 16.0 & 27.0 \\ 
        fingerprint & grp & FA-FP-IR & 0 & 9.0 & 18.0 \\ 
        fingerprint & grp & FA-IR-FP & 0 & 9.0 & 17.0 \\ 
        fingerprint & grp & FP-FA-IR & 0 & 9.0 & 18.0 \\ 
        fingerprint & grp & FP-IR-FA & 0 & 9.0 & 18.0 \\ 
        fingerprint & grp & IR-FA-FP & 0 & 9.0 & 18.0 \\ 
        fingerprint & grp & IR-FP-FA & 0 & 9.0 & 17.0 \\ 
        iris & baseline & FA-IR & 0 & 23.0 & 61.0 \\ 
        iris & baseline & IR-FA & 0 & 23.0 & 54.0 \\ 
        iris & baseline & FP-IR & 0 & 23.0 & 56.99 \\ 
        iris & baseline & IR-FP & 0 & 24.0 & 51.0 \\ 
        iris & baseline & FA-FP-IR & 0 & 24.0 & 56.00 \\ 
        iris & baseline & FA-IR-FP & 0 & 24.0 & 56.00 \\ 
        iris & baseline & FP-FA-IR & 0 & 22.0 & 53.0 \\ 
        iris & baseline & FP-IR-FA & 0 & 25.0 & 57.99 \\ 
        iris & baseline & IR-FA-FP & 0 & 23.0 & 54.0 \\ 
        iris & baseline & IR-FP-FA & 0 & 24.0 & 54.0 \\ 
        iris & biohashing & FA-IR & 0 & 25.0 & 56.00 \\ 
        iris & biohashing & IR-FA & 0 & 21.0 & 56.99 \\ 
        iris & biohashing & FP-IR & 0 & 22.0 & 63.0 \\ 
        iris & biohashing & IR-FP & 0 & 23.0 & 55.00 \\ 
        iris & biohashing & FA-FP-IR & 0 & 23.0 & 51.0 \\ 
        iris & biohashing & FA-IR-FP & 0 & 23.0 & 56.00 \\ 
        iris & biohashing & FP-FA-IR & 0 & 23.0 & 65.0 \\ 
        iris & biohashing & FP-IR-FA & 0 & 23.0 & 56.00 \\ 
        iris & biohashing & IR-FA-FP & 0 & 22.0 & 55.00 \\ 
        iris & biohashing & IR-FP-FA & 0 & 23.0 & 57.99 \\ 
        iris & grp & FA-IR & 0 & 19.0 & 54.0 \\ 
        iris & grp & IR-FA & 0 & 22.0 & 48.0 \\ 
        iris & grp & FP-IR & 0 & 19.0 & 50.0 \\ 
        iris & grp & IR-FP & 0 & 19.0 & 43.0 \\ 
        iris & grp & FA-FP-IR & 0 & 23.0 & 52.0 \\ 
        iris & grp & FA-IR-FP & 0 & 24.0 & 59.0 \\ 
        iris & grp & FP-FA-IR & 0 & 21.0 & 56.99 \\ 
        iris & grp & FP-IR-FA & 0 & 20.0 & 51.0 \\ 
        iris & grp & IR-FA-FP & 0 & 22.0 & 56.00 \\
        iris & grp & IR-FP-FA & 0 & 23.0 & 55.00 \\ 

        
    \bottomrule
	\end{tabular}
	\end{adjustbox}


